Toward Non-Invasive Diagnosis of Bankart Lesions with Deep Learning

Bankart lesions, or anterior-inferior glenoid labral tears, are diagnostically challenging on standard MRIs due to their subtle imaging features-often necessitating invasive MRI arthrograms (MRAs). This study develops deep learning (DL) models to detect Bankart lesions on both standard MRIs and MRAs, aiming to improve diagnostic accuracy and reduce reliance on MRAs. We curated a dataset of 586 shoulder MRIs (335 standard, 251 MRAs) from 558 patients who underwent arthroscopy. Ground truth labels were derived from intraoperative findings, the gold standard for Bankart lesion diagnosis. Separate DL models for MRAs and standard MRIs were trained using the Swin Transformer architecture, pre-trained on a public knee MRI dataset. Predictions from sagittal, axial, and coronal views were ensembled to optimize performance. The models were evaluated on a 20% hold-out test set (117 MRIs: 46 MRAs, 71 standard MRIs). Bankart lesions were identified in 31.9% of MRAs and 8.6% of standard MRIs. The models achieved AUCs of 0.87 (86% accuracy, 83% sensitivity, 86% specificity) and 0.90 (85% accuracy, 82% sensitivity, 86% specificity) on standard MRIs and MRAs, respectively. These results match or surpass radiologist performance on our dataset and reported literature metrics. Notably, our model's performance on non-invasive standard MRIs matched or surpassed the radiologists interpreting MRAs. This study demonstrates the feasibility of using DL to address the diagnostic challenges posed by subtle pathologies like Bankart lesions. Our models demonstrate potential to improve diagnostic confidence, reduce reliance on invasive imaging, and enhance accessibility to care.

==> sections/interpretability.tex <==
% GradCAM visualizations highlight regions relevant to a model's predictions.  \autoref{fig:grad_cam} presents Grad-CAM \cite{selvaraju_grad-cam_2017} visualizations for the axial view which highlight key regions that contributed to the model's predictions for Bankart lesion detection on both standard MRIs and MRAs. 

% \noindent \textbf{For the MRA}, the Grad-CAM visualization prominently highlighted a region in the posterior labrum that might initially suggest a reverse Bankart (posterior labral tear). However, based on the original radiology report and expert surgical annotation, this was determined to be a severe Bankart lesion where cartilage from the anterior-inferior labrum tore completely and translocated posteriorly. The highlighted region in the Grad-CAM output, which overlaps with the surgeon's annotation, reflects the area the model relied on for its decision. This alignment with the surgically verified region demonstrates the model’s capability to identify key pathological features, even in atypical cases.

% \noindent \textbf{For the standard MRI,} the Grad-CAM visualization
% %In contrast, the Grad-CAM visualization for the standard MRI 
% highlighted the anterior labrum, consistent with the region of interest for Bankart lesion detection. However, no obvious features indicative of a tear were visible to the annotating surgeon. This suggests that the model may detect subtle features not immediately evident to human observers, supporting its potential utility in challenging diagnostic contexts.

%    \begin{figure}[t]
%    \begin{center}
%    \begin{tabular}{c} %% tabular useful for creating an array of images 
%    \includegraphics[width=\textwidth]{Figures/resize_GradCAMFigure.pdf}
%    %[height=10cm]
%    %{Figures/GradCAMFigure.jpg}
%    \end{tabular}
%    \end{center}
%    \caption[example] 
% %>>>> use \label inside caption to get Fig. number with \autoref{}
%    { \label{fig:grad_cam} 
% Gradient-weighted class activation mapping (Grad-CAM)\cite{selvaraju_grad-cam_2017} visualizations for Bankart lesion detection on standard MRIs (left) and MRAs (right) on the axial view. The top row depicts cases with confirmed Bankart lesions, while the bottom row shows cases without tears. White circles highlight regions of interest annotated by a shoulder/elbow fellowship-trained orthopedic surgeon. For the MRA Bankart lesion case (top right), the model correctly identified a translocated piece of cartilage from the anterior labrum present near the posterior labrum, which was documented a Bankart lesion in the original radiology report and later verified in the surgical operative note. For the standard MRI Bankart lesion case (top left), the surgeon placed the circle in the region of the anterior labrum but noted that no clear tear was visible in the image. Heatmaps indicate regions most influential to the model’s prediction, with warmer colors (red/yellow) signifying higher relevance.}
%    \end{figure} 
% %-----Discussion:
% % The GradCAM visualizations highlight regions relevant to its predictions. I
% %n the MRA example, the model focused on a posteriorly translocated cartilage fragment, a unique presentation of an anterior Bankart lesion. This alignment with the surgically verified region demonstrates the model’s capability to identify key pathological features, even in atypical cases.

% % For the standard MRI, the model highlighted the anterior labrum, where no tear was clearly visible to the annotating surgeon. This suggests that the model may detect subtle features not immediately evident to human observers, supporting its potential utility in challenging diagnostic contexts.

% % These findings highlight the utility of visualization tools like Grad-CAM in examining model predictions and identifying regions of interest. 

==> sections/limitation_future_work.tex <==
% % Despite its promising results, this study has several limitations that warrant further investigation. One significant limitation 
% \textbf{Dataset Size:} A limitation of this study is the small number of positive cases in the test set (6/71, 8.45\%) for standard MRIs. This imbalance reflects current clinical practice, where standard MRIs are rarely ordered when a Bankart lesion is suspected due to their perceived lower diagnostic utility compared to MRI arthrograms. While our study aims to address this limitation of clinical practice by demonstrating the potential of deep learning to improve the utility of standard MRIs, additional studies with larger, more balanced, and multi-institution datasets are needed to validate our findings and strengthen their generalizability.

% \noindent \textbf{Reader Study:} A future 
% %Another critical area for future work is the incorporation of a 
% reader/observer study is critical to evaluate the model’s impact on clinical decision-making. The study would assess how clinicians interact with the model’s outputs, and compare clinician model-assisted and model-unassisted performance. This would assess the model’s practical utility and its potential to enhance diagnostic confidence and accuracy.

% \noindent\textbf{Model Interpretability: } Enhancing model interpretability is essential to facilitate clinical adoption \cite{barnett_case-based_2021}. Future work should explore using post-hoc interpretability techniques like GradCAM\cite{selvaraju_grad-cam_2017} on our existing models. Integrating interpretability techniques directly into the model should also be explored, such as the prototype-based \enquote{This Looks Like That} framework \cite{chen_this_2019}. This approach, which has been successfully applied in fields like breast cancer diagnosis \cite{barnett_case-based_2021}, enables models to reason through interpretable prototypes that align with clinically relevant features, potentially increasing trust and usability among clinicians.

% % Here, our interpretability efforts rely on the post-hoc tool GradCAM\cite{selvaraju_grad-cam_2017}, which, while useful, has inherent variability and limitations as it is heavily influenced by the optimization method, choice of model layer, and characteristics of the input images \cite{omeiza_smooth_2019, buono_expected_2024, lucas_visual_2022}. Grad-CAM is also susceptible to the gradient saturation problem, where important features may result in small gradient magnitudes, potentially misrepresenting feature importance \cite{omeiza_smooth_2019, buono_expected_2024, lucas_visual_2022}. Additionally,sensitivity to noise and the lack of standardized protocols for implementation can result in inconsistent or ambiguous heatmaps \cite{omeiza_smooth_2019, buono_expected_2024, lucas_visual_2022}. Therefore, while Grad-CAM can provide valuable insights into model behavior, its variability necessitates cautious interpretation. It is best utilized as a tool for approximate understanding rather than as a definitive mechanism for validating predictions.

% %Future work should explore i


% \noindent\textbf{Image Formats:} A transformative direction for this research lies in exploring techniques to convert standard MRIs into MRA-like images. This would be similar to the \enquote{virtual staining} approach that has shown success in digital histopathology \cite{latonen_virtual_2024}, and could enhance interpretability and usability for radiologists by creating synthetic MRA-like images that preserve the diagnostic familiarity of traditional arthrograms. However, this would be most feasible with paired standard MRI-MRA datasets, which may be challenging to acquire. Future work should investigate the feasibility of generating such datasets and the performance of models trained on these synthetic images.

==> tables/performance_across_folds.tex <==
%\FloatBarrier
\begin{table}[t]
\centering
\caption{Mean Cross-Validation AUC Across Folds}
%\renewcommand{\arraystretch}{1}  % Adjust row height for readability
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabular}{p{0.225\linewidth}>{\raggedright\arraybackslash}p{0.1\linewidth}>{\raggedright\arraybackslash}p{0.2\linewidth}>{\raggedright\arraybackslash}p{0.2\linewidth}}
\toprule
\textbf{View-Modality}& \textbf{AUC}&  \textbf{Standard Deviation (StDev)}&\textbf{95 \% Confidence Interval (CI)}\\
\midrule
Sagittal-Standard MRI& 0.759&  0.051& 0.716-0.801\\
Axial-Standard MRI& 0.729&   0.054& 0.684-0.775\\
Coronal-Standard MRI& 0.743&  0.038& 0.711-0.775\\
Sagittal-MRA& 0.770&  0.033& 0.742-0.798\\
Axial-MRA& 0.776&  0.028& 0.753-0.799\\
Coronal-MRA& 0.782&   0.026& 0.760-0.804\\
\bottomrule

\end{tabular}
%\vspace{5pt} % Add some space before footnotes
\parbox{0.85\textwidth}{%
\footnotesize%
% \textsuperscript{1} Standard Deviation \\
}
\label{tab:stability_across_folds}
\end{table}

